Diffusion framework for geometric and photometric data fusion in non-rigid shape analysis

In this paper, we explore the use of the diffusion geometry framework for the fusion of geometric and photometric information in local and global shape descriptors. Our construction is based on the definition of a diffusion process on the shape manifold embedded into a high-dimensional space where the embedding coordinates represent the photometric information. Experimental results show that such data fusion is useful in coping with different challenges of shape analysis where pure geometric and pure photometric methods fail.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

The amount of geometric data available in the public domain, such as Google 3D Warehouse, has grown dramatically  and created the demand for shape search and retrieval algorithms capable of finding similar shapes in the same way a search engine responds to text queries.
However, while text search methods are sufficiently developed to be ubiquitously used, the search and retrieval of 3D shapes remains a challenging problem. Shape retrieval based on text metadata, like annotations and tags added by the users, is often incapable of providing relevance level required for a reasonable user experience (see Figure \ref{fig:googles}).

\begin{figure}[t]
    \begin{center}
    \includegraphics*[width=1\linewidth,bb=1 1 986 619,clip]{img/GooGLeDog.png}
   \caption{ \small  The need for content-based shape retrieval: text-based search engine such as \textit{Google 3D Warehouse} returns shapes of dogs as well as hot-dog cabins in response to the query ``dog''. The later is obviously irrelevant. \label{fig:googles}}
    \end{center}
\end{figure}

\textit{Content-based shape retrieval} using the shape itself as a query and based on the comparison of 
geometric and topological properties of shapes is complicated by the fact that many 3D objects manifest rich variability, and shape retrieval must often be \textit{invariant} under different classes of transformations. A particularly challenging setting is the case of non-rigid shapes, including a wide range of transformations such as bending and articulated motion, rotation and translation, scaling, non-rigid deformation, and topological changes.
%
%
The main challenge in shape retrieval algorithms is computing a \textit{shape descriptor}, that would be unique for each shape, simple to compute and store, and invariant under different type of transformations. Shape similarity is determined by comparing the shape descriptors. Most of the current content-based shape retrieval methods use geometric properties of the shapes, such as intrinsic geometry structures, geodesics distances, local features etc., to create the shape descriptor.


Recently, there has been an increased interest in the use of {\em diffusion geometry} \cite{diff,levy2006lbe,reuter2009discrete} for constructing invariant shape descriptors.
Diffusion geometry is closely related to heat propagation properties of shapes and allows obtaining global structures, such as metrics, %\cite{bro-ghf},
%
%,BroBB1
distance distributions \cite{rustamov2007lbe,MS_GMOD} and spectral signatures \cite{reuter,reuter2009discrete}, as well local structures like
descriptors \cite{sunHKS} %,BroSI:HKS},
which are intrinsic %(\cite{reuter,reuter2009discrete}) and hence deformation invariant,
and hence deformation-invariant. %also scale - and topology - invariant (Figure \ref{fig:aikido}).
%
%{\bf ADD: [Sun ShapeGoogle] }
%In particular, heat kernel signatures \cite{sunHKS} showed very promising results in large-scale shape retrieval applications \cite{BroBroOvsGui09}.


One limitation of these methods is that, so far, only geometric information has been considered. However, in many cases, shapes come with \textit{photometric} information (texture). % like the texture seen in Figure \ref{fig:photom}.
Some recent papers demonstrated the use of both photometric and geometric information in shape analysis \cite{thorstensen}. %,chaohui:INRIA}.
%
%
More recently, Zaharescu \textit{et al.} \cite{zaharescu-surface} used photometric and geometric texture to build a 3D analogue of the SIFT descriptor \cite{low:IJCV:04} popular in computer vision.

{\bf More references!}

%Was defined \textit{discrete directional derivative, gradient} and \textit{discrete convolution}, then was build scale space for shape's scalar function (\textit{texture}) (by convolving it with Gaussian kernel) and then, in similar manner as for SIFT, found \textit{``interesting points''} and built descriptors.
%In similar manner this approach can be extended from image \textit{content-based-retrieval}(\cite{sift:retr}, \cite{sift:retr2}) to 3D shapes.

%\vspace{-.4cm}
%\begin{figure}[t]
%%\hspace{1cm}
%\begin{center}
%\label{fig:photom}
%\begin{minipage}[b]{0.39\linewidth}
%  \centering   \includegraphics*[width=0.6\linewidth,bb=1 1 401 651,clip]{img/adult_null.png}
%\end{minipage}
%%
%\begin{minipage}[b]{0.39\linewidth}
%  \centering     \includegraphics*[width=0.6\linewidth,bb=1 1 401 651,clip]{img/adult_null_photom.png}
%\end{minipage}
%%
%\end{center}
%  \caption{ Example of shape with geometric (left) and photometric (right) information.}
%\end{figure}

%%\vspace{-1.5cm}
%\begin{figure}[ht]
%    \begin{center}
%    \label{fig:aikido}
%    \includegraphics*[width=1\linewidth,bb=1 1 900 345]{img/SimAikido.png}
%   \caption{ \small Examples of similar textured shapes undergoing geometric and topological transformations. }
%    \end{center}
%\end{figure}

In this paper, we extend the diffusion geometry framework to include photometric information in addition to its geometric counterpart.
The main idea is to define a diffusion process that takes into consideration not only the geometry but also the texture of the shape.
As a result, we are able to construct local descriptors (heat kernel signatures) and global descriptors (diffusion distance distributions).
%
The proposed data fusion can be useful in coping with different challenges of shape analysis where pure geometric and pure photometric methods fail. %, e.g., topological noise, see Figure \ref{fig:fus1}.


%The rest of this paper is organized as follows. In Section~\ref{sec:backgr}, we review the mathematical formalism of diffusion processes and their use in shape analysis.
%In Section~\ref{sec:chks}, we introduce our approach and in Section~\ref{sec:num} its numerical implementation details.
%Section~\ref{sec:res} presents experimental results. Finally, Section~\ref{sec:concl} concludes the paper.


==> perf/BoFS-10.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 90.00} & {\small 95.00} & {\small 96.67} & {\small 97.50} & {\small 96.00} \\
{\small\em Partial} & {\small 81.25} & {\small 74.38} & {\small 71.11} & {\small 64.48} & {\small 65.08} \\
%\hline
%{\small{\bf Average}} & {\small 86.11} & {\small 85.83} & {\small 85.31} & {\small 82.82} & {\small 82.26} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.75} & {\small 98.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 95.00} & {\small 96.67} & {\small 97.50} & {\small 98.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 96.00} & {\small 84.51} & {\small 76.53} & {\small 71.39} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 86.33} & {\small 81.62} & {\small 76.03} \\
%\hline
%{\small{\bf Average}} & {\small 100.00} & {\small 98.38} & {\small 94.00} & {\small 91.21} & {\small 89.10} \\
\hline
{\small\em Mixed} & {\small 86.67} & {\small 79.76} & {\small 76.17} & {\small 78.38} & {\small 71.81} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of BoFs with cHKS descriptors using fixed colorspace scaling factor ($w=0.1$). \label{tab:BoFS-10}}
\end{table}

==> perf/cBoFS.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 93.33} \\
\hline
{\small{\bf Geometric}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 97.04} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 87.75} & {\small 76.62} & {\small 69.47} & {\small 61.60} \\
{\small\em Brightness} & {\small 87.00} & {\small 72.00} & {\small 56.66} & {\small 46.90} & {\small 39.59} \\
{\small\em Hue} & {\small 9.95} & {\small 7.47} & {\small 6.18} & {\small 5.52} & {\small 5.02} \\
{\small\em Saturation} & {\small 13.34} & {\small 13.31} & {\small 10.99} & {\small 9.74} & {\small 8.85} \\
{\small\em Noise} & {\small 100.00} & {\small 95.00} & {\small 88.33} & {\small 80.58} & {\small 74.74} \\
\hline
{\small{\bf Photometric}} & {\small 63.83} & {\small 56.07} & {\small 47.88} & {\small 42.29} & {\small 37.48} \\
\hline
{\small\em Mixed} & {\small 25.77} & {\small 25.49} & {\small 20.38} & {\small 18.39} & {\small 15.75} \\
\hline
\end{tabular}
\caption{\small Performance (mAP in \%) of color histograms. \label{tab:cBoFS}}
\end{table} 

==> perf/multi-resoliton-BoFS2.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 96.00} \\
{\small\em Partial} & {\small 68.75} & {\small 68.12} & {\small 69.03} & {\small 67.60} & {\small 67.58} \\
\hline
{\small{\bf Average}} & {\small 86.11} & {\small 85.83} & {\small 86.23} & {\small 85.60} & {\small 83.37} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 96.40} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of w-multi-scale BoFs with cHKS descriptors. \label{tab:multi-resolution-BoFS}}
\end{table}

==> perf/old/BoFS-0.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transform} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 96.67} & {\small 95.00} & {\small 90.00} \\
{\small\em Partial} & {\small 67.50} & {\small 67.50} & {\small 68.61} & {\small 67.08} & {\small 66.72} \\
\hline
%{\small{\bf Average}} & {\small 85.56} & {\small 85.56} & {\small 84.20} & {\small 82.59} & {\small 79.65} \\
%\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
%{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
%\hline
{\small\em Mixed} & {\small 90.00} & {\small 90.00} & {\small 93.33} & {\small 95.00} & {\small 96.00} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of ShapeGoogle using BoFs with HKS descriptors. \label{tab:BoFS-0}}
\end{table}

==> perf/old/BoFS-10.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 90.00} & {\small 95.00} & {\small 96.67} & {\small 97.50} & {\small 96.00} \\
{\small\em Partial} & {\small 81.25} & {\small 74.38} & {\small 71.11} & {\small 64.48} & {\small 65.08} \\
\hline
{\small{\bf Average}} & {\small 86.11} & {\small 85.83} & {\small 85.31} & {\small 82.82} & {\small 82.26} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.75} & {\small 98.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 95.00} & {\small 96.67} & {\small 97.50} & {\small 98.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 95.83} & {\small 84.48} & {\small 76.72} & {\small 71.54} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 86.33} & {\small 81.62} & {\small 75.83} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 98.33} & {\small 93.99} & {\small 91.26} & {\small 89.12} \\
\hline
{\small\em Mixed} & {\small 86.67} & {\small 79.76} & {\small 76.17} & {\small 78.38} & {\small 71.81} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of BoFs with cHKS descriptors using fixed colorspace scaling factor ($w=0.1$). \label{tab:BoFS-10}}
\end{table}

==> perf/old/cBoFH.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transform.} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
%{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
%\hline
{\small\em Contrast} & {\small 100.00} & {\small 90.83} & {\small 80.30} & {\small 71.88} & {\small 63.95} \\
{\small\em Brightness} & {\small 88.33} & {\small 80.56} & {\small 65.56} & {\small 53.21} & {\small 44.81} \\
{\small\em Hue} & {\small 11.35} & {\small 8.38} & {\small 6.81} & {\small 6.05} & {\small 5.49} \\
{\small\em Saturation} & {\small 17.47} & {\small 14.57} & {\small 12.18} & {\small 10.67} & {\small 9.74} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 93.33} & {\small 85.00} & {\small 74.70} \\
\hline
%{\small{\bf Average}} & {\small 65.37} & {\small 60.04} & {\small 52.03} & {\small 45.32} & {\small 39.65} \\
%\hline
{\small\em Mixed} & {\small 28.07} & {\small 25.99} & {\small 20.31} & {\small 17.62} & {\small 15.38} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of color histograms. \label{tab:cBoFH}}
\end{table}

==> perf/old/cBoFS.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 93.33} \\
\hline
{\small{\bf Geometric}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 97.04} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 87.75} & {\small 76.62} & {\small 69.47} & {\small 61.60} \\
{\small\em Brightness} & {\small 87.00} & {\small 72.00} & {\small 56.66} & {\small 46.90} & {\small 39.59} \\
{\small\em Hue} & {\small 9.95} & {\small 7.47} & {\small 6.18} & {\small 5.52} & {\small 5.02} \\
{\small\em Saturation} & {\small 13.34} & {\small 13.31} & {\small 10.99} & {\small 9.74} & {\small 8.85} \\
{\small\em Noise} & {\small 100.00} & {\small 95.00} & {\small 88.33} & {\small 80.58} & {\small 74.74} \\
\hline
{\small{\bf Photometric}} & {\small 63.83} & {\small 56.07} & {\small 47.88} & {\small 42.29} & {\small 37.48} \\
\hline
{\small\em Mixed} & {\small 25.77} & {\small 25.49} & {\small 20.38} & {\small 18.39} & {\small 15.75} \\
\hline
\end{tabular}
\caption{\small Performance (mAP in \%) of color histograms. \label{tab:cBoFS}}
\end{table} 

==> perf/old/multi-resoliton-BoFS.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transform.} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 96.67} & {\small 97.50} & {\small 94.00} \\
{\small\em Partial} & {\small 68.75} & {\small 68.12} & {\small 69.03} & {\small 67.60} & {\small 67.58} \\
\hline
%{\small{\bf Average}} & {\small 86.11} & {\small 85.83} & {\small 84.38} & {\small 84.21} & {\small 82.26} \\
%\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
%{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
%\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of ShapeGoogle using w-multi-scale BoFs with cHKS descriptors. \label{tab:multi-resolution-BoFS}}
\end{table}

==> perf/old/multi-resoliton-BoFS2.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 96.00} \\
{\small\em Partial} & {\small 68.75} & {\small 68.12} & {\small 69.03} & {\small 67.60} & {\small 67.58} \\
\hline
{\small{\bf Average}} & {\small 86.11} & {\small 85.83} & {\small 86.23} & {\small 85.60} & {\small 83.37} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 96.40} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of w-multi-scale BoFs with cHKS descriptors. \label{tab:multi-resolution-BoFS}}
\end{table}

==> perf/old/w-0,heat.l2-1024-4096-l1n-sum.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 80.00} & {\small 90.00} & {\small 88.89} & {\small 86.67} & {\small 89.33} \\
{\small\em Partial} & {\small 68.75} & {\small 71.88} & {\small 64.86} & {\small 61.15} & {\small 63.08} \\
\hline
{\small{\bf Average}} & {\small 75.00} & {\small 81.94} & {\small 78.21} & {\small 75.32} & {\small 77.67} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small\em Mixed} & {\small 90.00} & {\small 90.00} & {\small 90.00} & {\small 89.17} & {\small 88.67} \\
\end{tabular}
\caption{\small Performance (mAP in \%) of pure geometric spectral shape distance (\ref{eq:spec-dist-photo}). \label{tab:regular:diff}}
\end{table} 

==> perf/old/w-0,heat.l2-1024-l1n-null.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 75.00} & {\small 87.50} & {\small 86.67} & {\small 87.50} & {\small 88.00} \\
{\small\em Partial} & {\small 63.33} & {\small 75.42} & {\small 72.78} & {\small 68.65} & {\small 68.25} \\
\hline
{\small{\bf Average}} & {\small 69.81} & {\small 82.13} & {\small 80.49} & {\small 79.12} & {\small 79.22} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small\em Mixed} & {\small 85.00} & {\small 85.00} & {\small 85.00} & {\small 85.00} & {\small 85.00} \\
\\
\hline
\end{tabular}
\caption{\small Performance of heat.l2-1024-l1n-null (mAP in \%). \label{tab:Art_LB_Belkin_1Ring_exp_Sigma_2_WColor_0_LocalScale_0_FCol_xxx_PreCluster_0_AdoptW_0_1  1  1_1  1  1-heat.l2-1024-l1n-null}}
\end{table}

==> perf/old/w-10,heat.l2-1024-4096-l1n-sum.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 67.50} & {\small 65.00} & {\small 62.78} & {\small 60.10} & {\small 60.58} \\
\hline
{\small{\bf Average}} & {\small 85.56} & {\small 84.44} & {\small 83.46} & {\small 82.27} & {\small 82.48} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 96.67} & {\small 94.58} & {\small 93.33} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 85.58} & {\small 75.81} & {\small 70.00} & {\small 65.36} \\
{\small\em Noise} & {\small 100.00} & {\small 90.00} & {\small 81.33} & {\small 68.55} & {\small 56.42} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 95.15} & {\small 90.79} & {\small 87.22} & {\small 83.98} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 84.76} & {\small 78.51} & {\small 79.60} & {\small 70.61} \\
\\
\hline
\end{tabular}
\caption{\small Performance of heat.l2-1024-4096-l1n-sum (mAP in \%). \label{tab:Art_LB_Belkin_1Ring_exp_Sigma_2_WColor_0.1_LocalScale_0_FCol_xxx_PreCluster_0_AdoptW_0_1  1  1_1  1  1-heat.l2-1024-4096-l1n-sum}}
\end{table}

==> perf/old/w-mltsc,heat.l2-1024-4096-l1n-sum.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transform.} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 64.58} & {\small 73.96} & {\small 66.67} & {\small 63.02} & {\small 67.92} \\
\hline
%{\small{\bf Geometric}} & {\small 84.26} & {\small 88.43} & {\small 85.19} & {\small 83.56} & {\small 85.74} \\
%\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
%{\small{\bf Photometric}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
%\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 96.44} \\
\end{tabular}
\caption{\small Performance of (mAP in \%) of the multiscale joint geometric-photometric spectral distance (\ref{eq:spec-dist-joint}). \label{tab:mltsc-sum}}
\end{table} 

==> perf/w-0,heat.l2-1024-l1n-null.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transform.} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 75.00} & {\small 87.50} & {\small 86.67} & {\small 87.50} & {\small 88.00} \\
{\small\em Partial} & {\small 63.33} & {\small 75.42} & {\small 72.78} & {\small 68.65} & {\small 68.25} \\
\hline
{\small{\bf Average}} & {\small 69.81} & {\small 82.13} & {\small 80.49} & {\small 79.12} & {\small 79.22} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
\hline
{\small\em Mixed} & {\small 85.00} & {\small 85.00} & {\small 85.00} & {\small 85.00} & {\small 85.00} \\
\\
\hline
\end{tabular}
\caption{\small Performance of heat.l2-1024-l1n-null (mAP in \%). \label{tab:Art_LB_Belkin_1Ring_exp_Sigma_2_WColor_0_LocalScale_0_FCol_xxx_PreCluster_0_AdoptW_0_1  1  1_1  1  1-heat.l2-1024-l1n-null}}
\end{table}

==> perf/w-10,heat.l2-1024-4096-l1n-sum.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 67.50} & {\small 65.00} & {\small 62.78} & {\small 60.10} & {\small 60.58} \\
\hline
{\small{\bf Average}} & {\small 85.56} & {\small 84.44} & {\small 83.46} & {\small 82.27} & {\small 82.48} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 96.67} & {\small 94.58} & {\small 93.33} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 85.58} & {\small 75.81} & {\small 70.00} & {\small 65.36} \\
{\small\em Noise} & {\small 100.00} & {\small 90.00} & {\small 81.33} & {\small 68.55} & {\small 56.42} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 95.15} & {\small 90.79} & {\small 87.22} & {\small 83.98} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 84.76} & {\small 78.51} & {\small 79.60} & {\small 70.61} \\
\\
\hline
\end{tabular}
\caption{\small Performance of heat.l2-1024-4096-l1n-sum (mAP in \%). \label{tab:Art_LB_Belkin_1Ring_exp_Sigma_2_WColor_0.1_LocalScale_0_FCol_xxx_PreCluster_0_AdoptW_0_1  1  1_1  1  1-heat.l2-1024-4096-l1n-sum}}
\end{table}

==> perf/zaharescu/norm-zhBOFH-vocab1300.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 90.00} & {\small 88.33} & {\small 92.22} & {\small 91.67} & {\small 93.33} \\
{\small\em Partial} & {\small 100.00} & {\small 87.50} & {\small 87.50} & {\small 86.46} & {\small 85.17} \\
\hline
{\small{\bf Average}} & {\small 94.44} & {\small 87.96} & {\small 90.12} & {\small 89.35} & {\small 89.70} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 93.29} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.16} \\
\hline
{\small\em Mixed} & {\small 90.00} & {\small 90.00} & {\small 84.44} & {\small 84.05} & {\small 77.74} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFH-vocab1300.mat (mAP in \%). \label{tab:-BOFH-vocab1300.mat}}
\end{table}

==> perf/zaharescu/norm-zhBOFH-vocab48.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 83.33} & {\small 68.75} & {\small 70.83} & {\small 71.88} & {\small 71.67} \\
\hline
{\small{\bf Average}} & {\small 92.59} & {\small 86.11} & {\small 87.04} & {\small 87.50} & {\small 87.41} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Noise} & {\small 100.00} & {\small 95.00} & {\small 93.33} & {\small 90.00} & {\small 86.13} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 99.38} & {\small 99.17} & {\small 98.75} & {\small 98.02} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 95.00} & {\small 90.00} & {\small 84.17} & {\small 77.87} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFH-vocab48.mat (mAP in \%). \label{tab:-BOFH-vocab48.mat}}
\end{table}

==> perf/zaharescu/norm-zhBOFH-vocab850.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Partial} & {\small 100.00} & {\small 85.42} & {\small 86.11} & {\small 86.46} & {\small 86.67} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 93.52} & {\small 93.83} & {\small 93.98} & {\small 94.07} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 94.13} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.27} \\
\hline
{\small\em Mixed} & {\small 86.67} & {\small 88.33} & {\small 84.44} & {\small 84.17} & {\small 77.47} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFH-vocab850.mat (mAP in \%). \label{tab:-BOFH-vocab850.mat}}
\end{table}

==> perf/zaharescu/norm-zhBOFS-vocab1300.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 95.00} & {\small 96.67} & {\small 94.17} & {\small 95.33} \\
{\small\em Partial} & {\small 56.25} & {\small 51.70} & {\small 63.63} & {\small 68.56} & {\small 69.01} \\
\hline
{\small{\bf Average}} & {\small 80.56} & {\small 75.76} & {\small 81.99} & {\small 82.79} & {\small 83.64} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.33} & {\small 95.17} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 90.00} & {\small 80.83} & {\small 75.33} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 98.75} & {\small 97.19} & {\small 95.46} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 92.92} & {\small 82.40} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFS-vocab1300.mat (mAP in \%). \label{tab:-BOFS-vocab1300.mat}}
\end{table}

==> perf/zaharescu/norm-zhBOFS-vocab48.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 95.00} & {\small 96.67} & {\small 94.17} & {\small 95.33} \\
{\small\em Partial} & {\small 75.00} & {\small 61.15} & {\small 69.93} & {\small 68.28} & {\small 68.79} \\
\hline
{\small{\bf Average}} & {\small 88.89} & {\small 79.96} & {\small 84.79} & {\small 82.66} & {\small 83.54} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.33} & {\small 94.17} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.75} & {\small 99.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 88.89} & {\small 83.33} & {\small 78.33} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 98.61} & {\small 97.19} & {\small 95.33} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 93.33} & {\small 83.40} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFS-vocab48.mat (mAP in \%). \label{tab:-BOFS-vocab48.mat}}
\end{table}

==> perf/zaharescu/norm-zhBOFS-vocab850.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 95.00} & {\small 96.67} & {\small 94.17} & {\small 95.33} \\
{\small\em Partial} & {\small 55.00} & {\small 51.04} & {\small 63.19} & {\small 65.10} & {\small 66.25} \\
\hline
{\small{\bf Average}} & {\small 80.00} & {\small 75.46} & {\small 81.79} & {\small 81.25} & {\small 82.41} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.33} & {\small 94.17} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 93.33} & {\small 83.33} & {\small 76.67} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 99.17} & {\small 97.50} & {\small 95.38} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 96.67} & {\small 91.67} & {\small 81.40} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFS-vocab850.mat (mAP in \%). \label{tab:-BOFS-vocab850.mat}}
\end{table}

==> perf/zaharescu/unnorm-zhBOFH-vocab48.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transform.} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 95.00} & {\small 96.67} & {\small 94.17} & {\small 95.33} \\
{\small\em Partial} & {\small 75.00} & {\small 61.15} & {\small 69.93} & {\small 68.28} & {\small 68.79} \\
\hline
%{\small{\bf Average}} & {\small 88.89} & {\small 79.96} & {\small 84.79} & {\small 82.66} & {\small 83.54} \\
%\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.33} & {\small 94.17} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.75} & {\small 99.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 88.89} & {\small 83.33} & {\small 78.33} \\
%\hline
%{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 98.61} & {\small 97.19} & {\small 95.33} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 93.33} & {\small 83.40} \\
%\\
%\hline
\end{tabular}
\caption{\small Performance of BOFS-vocab48.mat (mAP in \%). \label{tab:-BOFS-vocab48.mat}}
\end{table}

==> perf/zaharescu/unnorm-zhBOFH-vocab850.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 65.00} & {\small 73.75} & {\small 65.00} & {\small 60.62} & {\small 58.00} \\
{\small\em Partial} & {\small 78.13} & {\small 44.83} & {\small 41.23} & {\small 44.90} & {\small 38.35} \\
\hline
{\small{\bf Average}} & {\small 70.83} & {\small 60.90} & {\small 54.43} & {\small 53.63} & {\small 49.27} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 94.13} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.27} \\
\hline
{\small\em Mixed} & {\small 64.50} & {\small 55.86} & {\small 52.81} & {\small 55.62} & {\small 48.64} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFH-vocab850.mat (mAP in \%). \label{tab:-BOFH-vocab850.mat}}
\end{table}

==> perf/zaharescu/unnorm-zhBOFS-vocab850.mat.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\bf\small Strength} \\
\cline{2-6}
{\bf\small Transformation} & {\bf\small 1} & {\bf\small $\leq$2} & {\bf\small $\leq$3} & {\bf\small $\leq$4} & {\bf\small $\leq$5}\\
\hline
{\small\em Isom+Topo} & {\small 100.00} & {\small 95.00} & {\small 96.67} & {\small 94.17} & {\small 95.33} \\
{\small\em Partial} & {\small 55.00} & {\small 51.04} & {\small 63.19} & {\small 65.10} & {\small 66.25} \\
\hline
{\small{\bf Average}} & {\small 80.00} & {\small 75.46} & {\small 81.79} & {\small 81.25} & {\small 82.41} \\
\hline
{\small\em Contrast} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 98.33} & {\small 94.17} \\
{\small\em Brightness} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 99.00} \\
{\small\em Hue} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Saturation} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} \\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 93.33} & {\small 83.33} & {\small 76.67} \\
\hline
{\small{\bf Average}} & {\small 100.00} & {\small 100.00} & {\small 99.17} & {\small 97.50} & {\small 95.38} \\
\hline
{\small\em Mixed} & {\small 100.00} & {\small 100.00} & {\small 96.67} & {\small 91.67} & {\small 81.40} \\
\\
\hline
\end{tabular}
\caption{\small Performance of BOFS-vocab850.mat (mAP in \%). \label{tab:-BOFS-vocab850.mat}}
\end{table}
